BiasConnect: Investigating Bias Interactions in Text-to-Image Models

The biases exhibited by Text-to-Image (TTI) models are often treated as if they are independent, but in reality, they may be deeply interrelated. Addressing bias along one dimension, such as ethnicity or age, can inadvertently influence another dimension, like gender, either mitigating or exacerbating existing disparities. Understanding these interdependencies is crucial for designing fairer generative models, yet measuring such effects quantitatively remains a challenge. In this paper, we aim to address these questions by introducing BiasConnect, a novel tool designed to analyze and quantify bias interactions in TTI models. Our approach leverages a counterfactual-based framework to generate pairwise causal graphs that reveals the underlying structure of bias interactions for the given text prompt. Additionally, our method provides empirical estimates that indicate how other bias dimensions shift toward or away from an ideal distribution when a given bias is modified. Our estimates have a strong correlation (+0.69) with the interdependency observations post bias mitigation. We demonstrate the utility of BiasConnect for selecting optimal bias mitigation axes, comparing different TTI models on the dependencies they learn, and understanding the amplification of intersectional societal biases in TTI models.

==> sec/3_Approach.tex <==
\section{Approach}
\label{sec:Approach}

\begin{figure*}
  \centering
   \includegraphics[width=\linewidth]{fig/main-approach.pdf}
   \caption{\textbf{An overview of \modelname}. We utilize a counterfactual based approach to measure pairwise causality between any two bias axes. For the axes that are dependent, we measure the causal effect, giving us an estimate of how bias mitigation along one axis impacts another}
   \label{fig:approach}
   % \vspace{-0.2cm}
\end{figure*}

The objective of \modelname\ is to quantify the dependencies between different bias dimensions in generative AI models by systematically altering input prompts and analyzing the resulting distributions of generated images. To achieve this, we generate counterfactual prompts by modifying specific bias attributes (e.g., gender, race, age) and examine how these interventions impact other bias dimensions. The key idea is that if modifying one bias axis (\(B_x\)) causes significant shifts in another bias axis (\(B_y\)), this indicates a dependency between these dimensions.

We frame this analysis as a \textbf{pairwise causal discovery problem}, where we test conditional independence between bias dimensions using Chi-square (\(\chi^2\)) tests. Specifically, we compute contingency matrices that capture the distributional shifts in \(B_y\) for different counterfactual versions of \(B_x\). By applying conditional independence tests, we construct a \textbf{pairwise causal graph} that reveals which bias dimensions influence each other (Sec.\ref{sec:Approach:CausalDiscovery}). This perspective aligns with the \textbf{interventional} level of Pearl’s \textit{Ladder of Causality}. Finally, we compute the causal treatment effect, defined as \isscore, by  along each bias dimension to measure its sensitivity to interventions on other dimensions, providing a structured evaluation of bias entanglement in generative AI models (Sec.\ref{sec:Approach:CausalEffect}). 



%Overall our approach is summarized as follows. For a given prompt $p$ and bias axes $B = [B_1, B_2... B_n]$, we first start by generating counterfactuals ($B_i$ can have counterfactuals $\{CF_i^1... CF_i^j\}$) across all bias axes, using templates defined in Supp. Sec. X. These prompts are then used to generate images via text-to-image (TTI) models, from which a VQA system extracts bias-related attributes. We then quantify pairwise causal relationships between bias axes to assess their dependencies. Finally, we compute the Causal Treatment Effect (CTE) along each bias dimension to measure its sensitivity to interventions on other dimensions, providing a structured evaluation of bias entanglement in generative AI models.


\subsection{Counterfactual Prompt-Image pair generation}
\label{sec:Approach:Imggen}
Given an input prompt $P$ and bias axes $B = [B_1, B_2... B_n]$, we first start by generating counterfactual prompts ($B_i$ can have counterfactuals $\{CF_i^1... CF_i^j\}$) across all bias axes, using templates defined in Supp. Sec. X. The original prompt $P$ and all counterfactuals 
%$\{CF_i^1... CF_i^j\}$ [no need to repeat this]
are then passed through a TTI model which generates images for all the prompts.

\subsection {VQA based bias information extraction}
\label{sec:Approach:VQA}
%As mentioned earlier, the primary motivation for using counterfactuals is to measure how intervening on $P$ along a given bias axis $B_K$, influences other bias axes $B_M$, where $B_M=B \slash B_K$. This comparison helps assess whether the bias introduced by modifying one axis also affects other bias dimensions. 
To facilitate a comparison among images generated by different prompts, we propose a VQA based concept-extractor. This module can leverage any existing framework or model designed for image set comparisons. Following previous approaches on bias evaluation like TIBET \cite{chinchure2024tibet} and OpenBias \cite{d2024openbias}, we employ a VQA based format to extract bias related concepts from the generated image counterfactual pairs. We use MiniGPT-v2 \cite{chen2023minigptv2} in a question-answer format to extract information from generated images. 

To reduce the impact of hallucination, we first use VQA to filter images that do not have a human in them. This is a small percentage of images that are ignored. Then, we have a list of predefined questions (Supp. X) corresponding to each bias axis in $B$, and each question has a choice of attributes to choose from. For example, for the gender bias axis, we ask the question ``\texttt{\small [vqa] What is the gender (male, female) of the person?}''. Note that every question is multiple choice (in this example, \texttt{\small male} and \texttt{\small female} are the two attributes for gender). The set of questions asked for all the images of prompt $P$
%$p$ 
and its counterfactuals $CF_i^j$ remain the same.


\subsection{Pairwise Causal Discovery}
\label{sec:Approach:CausalDiscovery}

Given an initial set of bias dimensions, the next step in our process involves constructing a causal graph. The algorithm begins by creating a complete undirected graph, where each bias dimension (e.g., gender, race, age) is connected to every other dimension by an edge. To refine this structure, we apply conditional independence tests using the Chi-square (\(\chi^2\)) test, systematically pruning edges between variables. Specifically, if two variables, \(X\) and \(Y\), are found to be conditionally independent given a conditioning set \(Z\), the edge between \(X\) and \(Y\) is removed. This conditional independence is expressed as 
\begin{math}
    X \perp Y \mid Z
\end{math},
\noindent where \(\perp\) denotes statistical independence. The result of this process is a skeleton graph that represents the potential causal relationships between bias dimensions.

For every pair of biases (\(B_x\),\(B_y\)) in the set \(B\), we compute a contingency matrix for the directed relationship \(B_x \to B_y\). This is done by counting the attributes of \(B_y\) across different counterfactual instances of \(B_x\). The Chi-square test is then used to assess the conditional independence between \(B_x\) and \(B_y\), with a threshold applied to the p-value for determining significant relationships. By repeating this test for all bias pairs in \(B\), we construct a pairwise causal graph.




%Future extensions of this work could incorporate edge orientation techniques, explicit confounder adjustments, and structured causal modeling to derive a more complete causal understanding of bias interactions in generative AI systems.
%\PS{this section will go down in the limitations section, but I want all the faculties to take look so that to ensure that we are making the right claims}


\subsection{Causal Treatment Effect Estimation}
\label{sec:Approach:CausalEffect}

When constructing a directed graph representing bias dependencies, using \(\chi^2\) weights can quantify the strength of dependence between different bias axes. However, the Chi-square statistic alone does not provide insight into whether the impact of \(B_x\) on \(B_y\) is positive or negative in terms of distributional shift towards an ideal distribution. This limitation arises because there is no direct comparison to the initial distribution of \(B_y\) in the original set of images generated from prompt \(p\). To address this, we propose a metric that quantifies the impact of bias mitigation on dependent biases with respect to an ideal distribution.  We estimate the effect of mitigation without actually conducting the mitigation step itself, and later verify that our estimate is valid.

\noindent{\bf Defining an Ideal Distribution.} We first define a desired (ideal) distribution, \(D^*\), which represents the unbiased state we want bias axes to achieve. This can be a real-world distribution of a particular bias axis, a uniform distribution (which we use in our experiments), or anything that suits the demographic of a given sub-population.
%\begin{itemize}
%    \item A real-world distribution of a particular bias axis.
%    \item A uniform distribution, which we use in our experiments.
%    \item Anything that suits the demographic of a given sub-population.
%\end{itemize}

\noindent{\bf Measuring Initial Bias Deviation.} Given the images of initial prompt \(p\), we compute the empirical distribution of attributes associated with bias axis \(B_y\), denoted as \( D_{B_y}^{\text{init}} \). We then compute the Wasserstein distance between this empirical distribution and the ideal distribution:

\begin{equation}
w_{B_y}^{\text{init}} = W_1(D_{B_y}^{\text{init}}, D^*)
\end{equation}

\noindent where \( W_1(\cdot, \cdot) \) represents the Wasserstein-1 distance. The Wasserstein-1 distance (also known as the Earth Mover's Distance) between two probability distributions \( D_1 \) and \( D_2 \) is defined as:

\begin{equation}
W_1(D_1, D_2) = \inf_{\gamma \in \Pi(D_1, D_2)} \mathbb{E}_{(x,y) \sim \gamma} [|x - y|]
\end{equation}

\noindent where \( \Pi(D_1, D_2) \) is the set of all joint distributions \( \gamma(x, y) \) whose marginals are \( D_1 \) and \( D_2 \), and \( |x - y| \) represents the transportation cost between points in the two distributions.

\noindent{\textbf{Intervening on $\mathbf{B_x}$.}}
Next, we intervene on \(B_x\). This intervention ensures that all counterfactuals of \(B_x\) are equally represented in the generated images. For example, if \(B_x\) represents gender bias, we enforce equal proportions of male and female individuals in the dataset. This is in line with most bias mitigation method proposed for TTI models, like ITI-GEN \cite{zhang2023iti}. After intervening by generating counterfactual along \(B_x\), we sum the distributions across all counterfactuals of \(B_x\) measured on \(B_y\), we obtain a new empirical distribution of \(B_y\), denoted as \( D_{B_y}^{B_x} \), and compute its Wasserstein distance from the ideal distribution:

\begin{equation}
w_{B_y}^{B_x} = W_1(D_{B_y}^{B_x}, D^*)
\end{equation}

\noindent{\textbf{Computing \isscore.}
To quantify the effect of mitigating \(B_x\) on \(B_y\), we define the metric, \isscore, as:

\begin{equation}
IS_{xy} = w_{B_y}^{\text{init}} - w_{B_y}^{B_x} 
\label{eqn:metric}
\end{equation}


%\noindent where:
%\begin{itemize}
    %\item \( IS_{xy} > 0 \) indicates that the estimated effect of mitigating \(B_x\) improves the distribution of \(B_y\), bringing it closer to the ideal distribution.
    %\item \( IS_{xy} < 0 \) indicates that the estimated effect of mitigating \(B_x\) has worsened the distribution of \(B_y\), moving it further from the ideal.
   % \item \( IS_{xy} = 0 \) means the the estimated effect of mitigating \(B_x\) had no impact on \(B_y\).
%\end{itemize}
\noindent where \( IS_{xy} \) quantifies the impact of mitigating bias \( B_x \) on bias \( B_y \). A positive value (\( IS_{xy} > 0 \)) indicates that mitigating \( B_x \) improves \( B_y \), bringing it closer to the ideal distribution, while a negative value (\( IS_{xy} < 0 \)) suggests it worsens \( B_y \), moving it further from the ideal. If \( IS_{xy} = 0 \), mitigating \( B_x \) has no effect on \( B_y \). This approach enables us to assess whether addressing one bias (e.g., gender) improves or worsens another (e.g., racial representation) in generative models, providing a systematic way to evaluate trade-offs and unintended consequences in bias mitigation strategies.


%This method allows us to quantify whether addressing one bias (e.g., gender) improves or worsens another bias (e.g., racial representation) in generative models. By applying this metric, we can systematically evaluate trade-offs and unintended consequences in bias mitigation strategies. 

\begin{figure*}[ht]
  \centering
   \includegraphics[width=\linewidth]{fig/examples.pdf}
   \caption{The figure illustrates bias interpretations from Bias Connects, combining all pairwise graphs into one. (a) Shows how mitigating clothing bias also mitigates emotion bias. (b) Explores interactions between non-traditional bias axes in the TIBET dataset. (c) Reveals that generating ethnically diverse athletes reduces gender diversity. (d) Demonstrates that diversifying salesperson clothing is best achieved by increasing ethnic diversity rather than directly specifying clothing variation.. }
   \label{fig:examples}
   % \vspace{-0.2cm}
\end{figure*}

\subsection{Visualizing as a Graph}

For the ease of visualization of readers, we present as graph (can also be an N by N matrix). It is a set of pairwise causal matrix.

The graph should be interpreted as follows:
For any focal node X, this is the node on which intervention is being done. You can consider every outgoing edges for X to observe causal effects from that node. \adi{WIP}

% \begin {itemize}
% \item Intro paragraph describing the approach in a holistic manner.
% \item Block Diagram Explaining our approach 
% \item Step 1- Counterfactual and Concept Extraction  

% \item Step 2- Contingency Table Creation 
% \item Step 3- Causal Discovery 
% \begin{itemize}
%         \item A paragraph that describes , the assumption and why this approach is causal 
%     \end{itemize}
% \item Step 4 - Causal Treatment Effect Estimation 
% \begin{itemize}
%         \item A paragraph that describes , the assumption and why this approach is causal 
%     \end{itemize}

% \end {itemize}

\section{Connection to Causality}
This section comments on causal aspect of our approach, where we justify the links between  our proposed approach to existing work in the causal literature
\subsection {Pairwise Causal Discovery}
\noindent{\bf Relationship with  PC algorithm.} Our approach corresponds to the first step of the well-known PC algorithm \cite{spirtes2000causation}, a foundational causal discovery method. However, we deliberately restrict ourselves to this initial step without further edge orientation. The reason for this choice is that our counterfactual generation process only considers a single level of intervention—measuring changes in \(B_y\) when \(B_x\) is altered. While full causal structure learning through edge orientation is theoretically possible, we observed that this process often leads to significant information loss regarding how different edges influence each other. Therefore, we prioritize preserving the richness of the pairwise relationships in the causal graph.

\noindent{\bf Causal Interpretation.}
This approach aligns with the \textbf{interventional} level of Pearl’s \textit{Ladder of Causality}, as we actively generate counterfactuals rather than passively observe existing data. However, it does not constitute \textbf{full causal inference}, as we do not explicitly control for confounders or orient edges to establish direct causal relationships. Unlike traditional causal modeling approaches that infer \textbf{global causal graphs}, our method focuses on \textbf{local, pairwise dependencies}, allowing us to detect how specific biases interact without assuming a fully specified causal model. 
A detailed explanation of restricted our approach to be pairwise causal instead of building a fully causal approach  with experiments has been provided in the Supplementary Material (Section \ref{sup:PC})


\subsection{ Causal Treatment Effect}
\noindent{\textbf{Causal Interpretation.}} This method can be framed as a \textbf{causal treatment effect} because it quantifies how mitigating one bias (\(\mathbf{B}_x\)) causally influences another bias (\(\mathbf{B}_y\)) through an intervention-based approach. By actively modifying \(\mathbf{B}_x\) (e.g., ensuring equal representation across its attributes) and measuring changes in the Wasserstein distance of \(\mathbf{B}_y\) from an ideal distribution, we estimate the causal impact of debiasing. This aligns with \textit{counterfactual causal inference} \cite{}, where we compare the observed outcome (\(\mathbf{B}_y\) distribution) with its hypothetical state had no intervention occurred. The method follows \textit{Rubin's causal model \cite{}}, treating bias mitigation as a \textit{treatment-control experiment}, and can be represented in a \textit{Directed Graph} as \( \mathbf{B}_x \to \mathbf{B}_y \), making it distinct from mere correlation analysis. The metric $BS_{xy}$ in Equation \ref{eqn:metric} captures the direction and magnitude of causal influence, providing insights into whether mitigating one bias improves or worsens another.



==> sec/6_Discussions.tex <==






\begin{figure*}
  \centering
   \includegraphics[width=\linewidth]{fig/tibet-egs.pdf}
   \caption{\textbf{Analyzing prompt-level impacts on the TIBET dataset using \modelname}. }
   \label{fig:tibetegs}
   % \vspace{-0.2cm}
\end{figure*}

==> sec/formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/oldnotes.tex <==

% \subsection{Bias Mitigation in TTI Models}
% \textbf{Dataset}: Proposed Dataset \\
% \textbf{Models}: Stable Diffusion 1.5 and 2.1

% \subsubsection{Experiment 1: Evaluating the Causal Discovery Approach}
% \begin{itemize}
%     \item \textbf{Aim}: Verify the effectiveness of the proposed causal discovery approach.
%     \item \textbf{Comparison Metrics}: 
%     \begin{itemize}
%         \item Bias Scores (Proposed Metric for Causal Treatment Effect Verification and MAD)
%         \item Image Quality
%         \item Algorithm Convergence Speed
%     \end{itemize}
%     \item \textbf{Methods}: 
%     \begin{itemize}
%         \item \textbf{Our Approach}
%         \item \textbf{Baselines}: 
%         \begin{itemize}
%             \item Randomized Nodes
%             \item Greedy Heuristic Algorithm
%             \item Metric evaluations on the original models
%         \end{itemize}
%         \item \textbf{Mitigation Strategies}: 
%         \begin{itemize}
%             \item Single-axis mitigation
%             \item Multi-axis mitigation (two, three, and all bias axes)
%         \end{itemize}
%     \end{itemize}
% \end{itemize}

% \subsubsection{Experiment 2: Evaluating Causal Treatment Effect Efficiency}
% \begin{itemize}
%     \item \textbf{Aim}: Assess the efficiency of the causal treatment effect approach.
%     \item \textbf{Dataset}: Proposed Dataset
%     \item \textbf{Models}: Stable Diffusion 1.4 and 2.1
%     \item \textbf{Procedure}: 
%     \begin{itemize}
%         \item Measure bias scores before and after applying the mitigation approach.
%         \item Compute Top-K Precision and Top-K Recall.
%         \item Analyze the correlation between predicted bias mitigation estimates and empirical outcomes.
%     \end{itemize}
% \end{itemize}

% \textbf{Datasets}: Proposed Dataset and TIBET Dataset (Design choices detailed in Appendix)

% \subsubsection{Comparison Across Different Models}
% \begin{itemize}
%     \item \textbf{Aim}: Understand underlying bias relationships between different Stable Diffusion models.
%     \item \textbf{Procedure}: 
%     \begin{itemize}
%         \item Generate a causal graph that includes all bias axes, all prompts, and all occupations.
%         \item Highlight key bias pathways with sample occupations.
%         \item Identify professions with the highest bias deviation across models.
%     \end{itemize}
% \end{itemize}

% \subsubsection{Comparison Across Different Bias Axes}
% \begin{itemize}
%     \item \textbf{Aim}: Identify bias axes with the greatest positive or negative impact on others.
%     \item \textbf{Procedure}: 
%     \begin{itemize}
%         \item Generate bubble charts, relationship graphs, or adjacency matrices to analyze proximity between bias axes.
%         \item Focus on key axes such as gender, age, and ethnicity across all models.
%     \end{itemize}
% \end{itemize}

% \section{Bias Mitigation in TTI models }
% \label{sec:bias_mitigation}

% \begin {itemize}
% \item Algorithm 
% \item Paragraph describing the LP Algorithm 
% \item Describe all the constraints to the LP algorithm 
% \end{itemize}

% %-------------------------------------------------------------------------



% \subsection{Causal Graph Verification}
% \textbf{Dataset}: Proposed Dataset \\
% \textbf{Model}: Stable Diffusion Family



% \subsubsection{VQA Sensitivity Analysis}
% \begin{itemize}
%     \item \textbf{Aim}: Estimate the sensitivity of the causal graph to noise in the VQA.
%     \item \textbf{Procedure}: 
%     \begin{itemize}
%         \item Systematically introduce errors in the VQA system.
%         \item Measure changes in the causal graph structure and causal treatment effect.
%     \end{itemize}
%     \item \textbf{Expected Outcome}: Minimal overall error in the causal graph and causal treatment effect.
% \end{itemize}

% \subsubsection{Sensitivity Analysis for Number of Images}
% \begin{itemize}
%     \item \textbf{Aim}: Assess the sensitivity of the causal graph to variations in dataset size.
%     \item \textbf{Procedure}: 
%     \begin{itemize}
%         \item Randomly subsample $k = 30\%, 40\%, 50\%, 80\%$ of the total dataset.
%         \item Analyze changes in the graph structure.
%         \item Compute the edit distance (change in the number of nodes) and graph variance.
%     \end{itemize}
% \end{itemize}

% \subsubsection{User Study}
% \begin{itemize}
%     \item \textbf{Aim}: Evaluate whether the counterfactuals generated by the model are intuitively meaningful to human users.
%     \item \textbf{Procedure}: Conduct a user study where participants assess the plausibility and coherence of generated counterfactuals.
% \end{itemize}

